Adaptive Model Selection Framework: An Application to Airline Pricing

Multiple machine learning and prediction models are often used for the same prediction or recommendation task. In our recent work, where we develop and deploy airline ancillary pricing models in an online setting, we found that among multiple pricing models developed, no one model clearly dominates other models for all incoming customer requests. Thus, as algorithm designers, we face an exploration - exploitation dilemma. In this work, we introduce an adaptive meta-decision framework that uses Thompson sampling, a popular multi-armed bandit solution method, to route customer requests to various pricing models based on their online performance. We show that this adaptive approach outperform a uniformly random selection policy by improving the expected revenue per offer by 43% and conversion score by 58% in an offline simulation.

==> sections/delete_me.tex <==
The online business performance of our deployed models is, on average, consistently better than human rule-based approaches. However, as is apparent, no one model dominates in performance, resulting in an erratic trend in in the revenue per offer among the models deployed online. This is due to a pre-configured standard A/B testing framework in the system of a real airline. The next question of interest, therefore, is a meta-learning approach that directs traffic efficiently to the right model for that session. 

We now model the traffic share value as a meta-parameter, which can then be tuned for targeting traffic more effectively to the better performing model. Learning this parameter is therefore critical to identify the ``winning'' model and separate it from other models. Based on customers' responses (to purchase an ancillary or not), we can reinforce the meta-parameters to adapt to the outcome. The multi-armed bandit approach is one such reinforcement learning technique that accomplishes this exact task.

\subsection{Multi-Armed Bandit Approach}
The multi-armed bandit problem is an extensively studied reinforcement learning technique which is widely used as a part of A/B testing. Solving this problem involves determining a sequence of decisions to choose from a given action space, with the reward associated with each action or `arm' only partially known (or having a random component). The environment (``nature'') reveals a reward after each action is taken, thereby also revealing more information about the random component of that action's reward. The objective of the problem is to maximize the expected rewards, i.e., minimize the cumulative expected regret. The bandit problem involves trade off between exploitation and exploration since the reward is only revealed for the chosen action. Hence, this problem setting makes if perfectly suitable for A/B testing. At each possible action step, the tradeoff made by the decision-maker is to exploit the action that has the highest expected tradeoff with the updated information available until that point, and to explore other actions to gather more information about the random component of the reward of those actions, to maximize gain in the long run. 

In our framework, each of the multiple models is viewed as an arm of the multi-armed bandit problem. This enables the decision-maker to direct online traffic based on the customer's response to the price offered by that arm. Hence, this meta-learning approach provides a trainable mechanism to allocate customer traffic to the arms during the test based on performance. Furthermore, meta-learning allows potentially different expected conversion rates of the different arms in an online setting. We explore one of the techniques to solve the multi-arm bandit problem, called Thompson Sampling , to allow us to exploit arms that have performed well in the past and explore seemingly inferior arms in case it might outperform the current winning arm. 

\subsection{Thompson Sampling for the Bernoulli Bandit}
In a Bernoulli bandit problem, there are a total of $A$ valid actions. An action $a_{t} \subseteq A$ at time $t$ produces a reward $r_{t} \in \{0, 1\}$ of one with probability $\theta_{a}$ and zero with probability $1 - \theta_{a}$. The mean reward $\theta = (\theta_{1}, \dots ,\theta_{A})$ is assumed to be unknown, but is constant over time. The agent begins with an independent prior belief over each $\theta_k$. As observations are gathered, the distribution is updated according to Bayes’ rule. The priors, according to equation \ref{eq:beta}, are assumed to be beta-distributed with parameters $\alpha_a \in \{\alpha_1, \dots , \alpha_A\}$ and $\beta_a \in \{\beta_1, \dots , \beta_A\}$. In particular, the exact prior probability density function given for an action $a$ is, 

\begin{equation}
\label{eq:beta}
p_{beta}(\theta_a) = \frac{\Gamma(\alpha_a + \beta_a)}{\Gamma(\alpha_a)\Gamma(\beta_a)} \theta_{a}^{(\alpha_a - 1)}(1-\theta_{a})^{(\beta_a - 1)}
\end{equation}

where $\Gamma$ denotes the gamma function. The beta distribution is particularly suited to this computation because it is a conjugate prior to the Bernoulli distribution.

\subsubsection{Simulation}
In this section we discuss an offline simulation performed on synthetic data to show the convergence rate of Thompson Sampling. Here, we have initialized three experimental models that have a success rate of $0.45$, $0.55$ and $0.60$. The aim of this simulation is to achieve this success rate through multi-armed bandit approach. The algorithm \ref{alg:ts} presents the pseudocode of the implementation used for simulation.  

\begin{algorithm}
\caption{Thompson Sampling for the Bernoulli Bandit}\label{algo:TS}
\label{alg:ts}
  \begin{algorithmic}[1]
    \FOR{$t = 1, 2, \dots$}
      \FOR{$a = 1, \dots, A$}
        \STATE Sample $\hat{\theta_a} \sim \text{Beta}(\alpha_a, \beta_a)$
      \ENDFOR
      \STATE $x_t \leftarrow$ $\argmax_a \hat{\theta_a}$ 
      \STATE Apply $x_t$
      \STATE Observe $r_t$
      \STATE $(\alpha_{x_t}, \beta_{x_t}) \leftarrow (\alpha_{x_t} + r_t, \beta_{x_t} + 1 - r_t)$
    \ENDFOR
  \end{algorithmic} 
\end{algorithm}

We start the simulation with the prior $\theta^{0} = Beta(\alpha=1, \beta=1)$, which corresponds to a uniform prior between 0 and 1. Note the initial uniform distribution can be seen in Figure \ref{fig:ts}. The run is then simulated for 2000 steps and target probabilities are recorded. In practice, the simulation results converged in approximately 1000 steps. Table \ref{tab:simulation} shows the convergence of the Thompson Sampling approach for the multi-armed bandit problem, demonstrating that the latent probability distribution can be inferred using this approach.   

\begin{table}[h]
\centering
\caption{Simulation results for Thompson Sampling}
\begin{tabular}{@{}cccc@{}}
\toprule
$\theta$ & True probability & Simulated probability & Trials \\ \midrule
$\theta_1$    & 0.45      & 0.45           & 70     \\
$\theta_2$    & 0.55      & 0.55           & 305    \\
$\theta_3$    & 0.60      & 0.61           & 1625   \\ \bottomrule
\end{tabular}
\label{tab:simulation}
\end{table}



\subsection{Constraints, Context and  Caution} \label{CCC}
Thompson sampling can be applied fruitfully to a broad array of online decision problems beyond the Bernoulli bandit. Thompson sampling outperforms other stochastic bandit algorithms (KL-UCB, Bayes UCB, UCB, $\epsilon$-greedy etc) on most bandit-type problems. But in problems involving time-varying constraints on the action, line 5 in Algorithm \ref{alg:ts} has to modified.

Another extension of the multi-armed bandit approach addresses contextual online decision problems. In these problems, the choice of the arm in a multi-armed bandit $a_t$ also depends on an independent random variable $z_t$ that the agent observes prior to making the decision. In such scenarios, the conditional distribution of the response $y_t$ is of the form $p_{\theta}(\cdot |a_t, z_t)$. Contextual bandit problems of this kind can be addressed through augmenting the action space and introducing time-varying constraint sets by viewing action and constraint together as $\tilde{a_t} = (a_t, z_t)$, with each arm (choice) represented as $\tilde{A_t} = \{(a_t,z_t : a\in A)\}$, where $A$ is the set from which $x_t$ must be chosen. After which it is straightforward to apply thompson sampling to select action. 

In certain situations when models have a particular baseline criteria to maintain, caution-based sampling can be used. This can be accomplished through constraining actions for each time $t^{th}$ step to have lower bound on expected average reward as $A_t = \{ a \in A : \mathbb{E}[r_t| a_t = a] \geq \tilde{r}\}$. This ensures that expected average reward at least exceeds $\tilde{r}$ using such actions. 

\subsection{Non-stationary systems and Concurrence} \label{Non stationary systems and Concurrence}
So far, we discussed settings in which model parameters $\theta$ are constant over time i.e. belong to a stationary system. In practice, the decision-maker could face a  non-stationary system, which is more appropriately modeled by time-varying parameters, such that reward is generated by $p_{\theta_t}(\cdot |a_t)$. In such contexts, the arm of the problem will never stop exploring, which could be a potential drawback. A more robust method involves ignoring all historical observations made prior to a certain time period $\tau$ in the past. Now, decision-makers produce a posterior distribution after every time step $t$ based on the prior and conditioned only on the most recent $\tau$ actions and observations. Model parameters are sampled from this distribution, and an action is selected to optimize the associated model. 

Dynamic pricing is one such problem where a single recommendation could be a weighted sum of recommendations from multiple arms, a concept referred to as concurrence. This is a case where the decision-maker takes multiple actions (arms) concurrently. Concurrency can be predefined with number of fixed arms to be pulled every time or it could be coupled with baseline caution (discussed in Section \ref{CCC}). This approach is similar to an approach based on an ensemble of models.

\subsection{Online implementation for ancillary pricing at Deepair} \label{Online implementation}
Although the assumption of models being temporally stable is a crucial assumption while using Thompson Sampling in multi-armed bandit settings, the offline simulations we performed for meta-learning provide reasonable evidence of convergence to the true distribution of the choice of models. Hence, our meta-learning approach shows promising offline results on synthetic data. For online deployment in the airline's systems, meta-learning using a multi-armed bandit approach can be used to route incoming customer bookings to each of the considered models, which serve as arms of the bandit. Additionally, meta-learning could also potentially handle concurrency by pricing using multiple models. Currently, meta-learning based models are being deployed to our partner airlines without concurrency being enabled, with the concurrency feature under development. Using targeted traffic routing, we hope to further improve our online metrics of evaluation as far as business value is considered. We are actively developing models that can improve the estimation accuracy. 
